Style Pooling: Automatic Text Style Obfuscation for Improved Classification Fairness

Text style can reveal sensitive attributes of the author (e.g. race or age) to the reader, which can, in turn, lead to privacy violations and bias in both human and algorithmic decisions based on text. For example, the style of writing in job applications might reveal protected attributes of the candidate which could lead to bias in hiring decisions, regardless of whether hiring decisions are made algorithmically or by humans. We propose a VAE-based framework that obfuscates stylistic features of human-generated text through style transfer by automatically re-writing the text itself. Our framework operationalizes the notion of obfuscated style in a flexible way that enables two distinct notions of obfuscated style: (1) a minimal notion that effectively intersects the various styles seen in training, and (2) a maximal notion that seeks to obfuscate by adding stylistic features of all sensitive attributes to text, in effect, computing a union of styles. Our style-obfuscation framework can be used for multiple purposes, however, we demonstrate its effectiveness in improving the fairness of downstream classifiers. We also conduct a comprehensive study on style pooling's effect on fluency, semantic consistency, and attribute removal from text, in two and three domain style obfuscation.

==> body/background.tex <==
\section{Background}
Probabilistic style transfer

==> body/excerpts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%


 \begin{figure*}
    \centering
        \begin{subfigure}{0.33\textwidth}
     \includegraphics[width=\linewidth]{figs/2dom-accuracy.pdf}
     \caption{2dom accuracy}
     \label{fig:blogs-2dom-acc}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
     \includegraphics[width=\linewidth]{figs/2dom-gpt.pdf}
     \caption{2dom gpt score}
     \label{fig:blogs-2dom-gpt}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
     \includegraphics[width=\linewidth]{figs/2dom-unc.pdf}
     \caption{2dom uncertainty}
     \label{fig:blogs-2dom-unc}
    \end{subfigure}
    
        \begin{subfigure}{0.33\textwidth}
     \includegraphics[width=\linewidth]{figs/3dom-accuracy.pdf}
     \caption{3dom accuracy}
     \label{fig:blogs-2dom-acc}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
     \includegraphics[width=\linewidth]{figs/3dom-gpt.pdf}
     \caption{3dom gpt score}
     \label{fig:blogs-2dom-gpt}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
     \includegraphics[width=\linewidth]{figs/3dom-unc.pdf}
     \caption{3dom uncertainty}
     \label{fig:blogs-2dom-unc}
    \end{subfigure}
    \caption{2dom and 3 dom blogs results}
    \label{fig:blogs}
    %\vspace{-1ex}
\end{figure*}
%%%%%%%%%%%%%%%%
%\begin{figure}
 %   \includegraphics[width=\linewidth]{figs/multi-domain.pdf}
 %   \caption{Synthesized}
 %   \label{fig:synthesized}
%\end{figure}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%

==> tables/2dom_temp.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
\begin{tabular}{@{}cDrrrrrrcrrrr@{}}
% \begin{tabular}{@{}DSSSSSSSSS@{}}
	\toprule
	%
	&\multirow{2}{*}{Metric} & \multirow{2}{*}{Original} & \multirow{2}{*}{A4NT}	&\multicolumn{3}{c}{One-LM}	 && \multicolumn{3}{c}{Inters.}	& \multirow{2}{*}{Union} \\
	\cmidrule[0.1pt]{5-7} \cmidrule[0.1pt]{9-11}  
	&                       &                            &                          & No DB & DB = 25 & DB = 40 && No DB & No DB hu& DB = 25  &  DB = 40  & \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{3}{*}{\STAB{Ling.}} & 
    BT Accuracy (\%)    &{100.00}	&66.49	&94.47	&92.88	&90.60	&&88.92	& 95.41 &87.39	&88.63	&96.88 \\
    %%%%%%%%%%&&&&&&&\\
    &GPT-2 PPL	        &41.71	&44.85	&39.51	&53.65	&66.21	&&36.14 & 41.6	&42.80	&58.15	&42.07\\
    %%%%%%%%%%&&&&&&&\\
    &Lex. Div. (\%)	    &3.22	&2.28	&2.52	&1.82	&1.09	&&2.28 & 2.50	&1.47	&0.97	&2.71\\
    %%%%%%%%%&&&&&&&\\
    \midrule[0.1pt]
    \multirow{3}{*}{\STAB{Clsf.}} &
    Clsf. Accuracy (\%)	&64.73	&61.31	&62.07	&61.69	&59.52	&&62.16 & 64.23	&60.90	&59.81	&64.02\\
    %%%%%%%%%%&&&&&&&\\
    &Entropy	            &0.87	&0.86	&0.87	&0.91	&0.95	&&0.87 & 0.87	&0.93	&0.95	&0.87\\
    %%%%%%%%%%%&&&&&&&\\
    &CR (\%)	            &14.21	&15.72	&13.44	&6.49	&2.80	&&12.25 & 13.95	&4.78	&2.47	&14.22\\
	%%%%%%%%%
	\bottomrule
\end{tabular}


==> tables/entropies.tex <==
 \newcolumntype{L}{>{\centering\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{O}{>{\centering\arraybackslash}m{0.08\linewidth}} 
  \newcolumntype{D}{>{\centering\arraybackslash}m{0.18\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
\begin{tabular}{@{}LLLLLLLLLL@{}}
	\toprule
	Domains & Original & A4NT & Sum LM & One LM & sum LM-25 &One LM-25 & Sum LM-40&	One LM-40&	Min LM \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
		2 Doms & 0.865&	0.856	&0.869	&0.865	&0.930&	0.914	&0.947	&0.945	&0.865	\\
	%%%%%%%%%
        3 Doms& 1.379&	-	&1.387	&1.380&	1.441	&1.431	&1.485	&1.468	&1.370\\
	%%%%%%%%%
	\bottomrule
\end{tabular}


==> tables/fairness_ratio.tex <==
\setlength{\tabcolsep}{1pt}% just a minimum
\begin{tabular*}{0.5\textwidth}{@{\extracolsep{\fill}}lllllll@{}}
\toprule
\multirow{2}{*}{Ratio} & \multicolumn{3}{c}{Occupation} & \multicolumn{3}{c}{TPR-Gap}  \\\cmidrule{2-4} \cmidrule{5-7} 
                        & Original     & A4NT       & Ours      & Original     & A4NT       & Ours     \\\midrule
$0.95$                  & 74.06        & 59.35      & 69.73     & 0.54         & 0.29       & 0.21                      \\
$0.80$                  &65.55	       &54.74	    &59.60      &0.35	       &0.21	    &0.18                \\
$0.65$                  &59.01	       &52.73	    &54.45	    &0.12	       &0.05	    &0.11                     \\
$0.50$                  &58.09	       &53.47	    &53.18	    &0.04	       &0.08	    &0.03                      \\\bottomrule

                          
\end{tabular*}

==> tables/fairness_ratio_comp.tex <==
% \setlength{\tabcolsep}{1pt}% just a minimum
\centering
\begin{tabular*}{0.94\textwidth}{@{}lSSSSScSSSSS@{}}
\toprule
\multirow{2}{*}{Ratio} & \multicolumn{5}{c}{Occupation Accuracy (Utility)} & & \multicolumn{5}{c}{TPR-gap (Fairness)}  \\\cmidrule{2-6} \cmidrule{8-12} 
                        & \text{Original}     & \text{A4NT}   &\text{Intrs.}      &\text{Intrs.
                        (DB)} &\text{Union} &   & \text{Original}     & \text{A4NT}   &\text{Intrs.}     & \text{Intrs. (DB)}  &\text{Union}\\\midrule
$0.95$                  & 74.56        & 59.35  &74.39       &69.73       &73.22 &       & 0.54         & 0.29   & 0.26          & 0.21     &0.51\\
$0.80$                  &65.55	       &54.74	&65.52       &59.60       &65.43 &       &0.35	        &0.21	 &0.34           &0.18      & 0.36\\
$0.65$                  &59.01	       &52.73	&57.59       &54.45       &57.19 &       &0.12	        &0.05	&0.12          &0.11       &0.15\\
$0.50$                  &58.09	       &53.47	&57.37       &53.18	      &55.49 &       &0.04	       &0.08	&0.05           &0.03        &0.05\\\bottomrule

%data for this table is in notion
                          
\end{tabular*}

==> tables/sentences.tex <==
 \newcolumntype{L}{>{\centering\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{O}{>{\centering\arraybackslash}m{0.08\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.28\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
\begin{tabular}{@{}lDDD@{}}
	\toprule
    Age &Input Sentence (Original Data)&A4NT& Proposed Method \\
	%%%%%%%%%
    \midrule
Teen&\textbf{grr} ... now i get cold quicker . & \textbf{grr} now i get cold \textbf{lol} . & \textbf{hmmm} ... now i get cold .   \\
Teen&it was so \textbf{fricken} hilarious .        & it was so ~\textbf{boring} hilarious .   &  it was so ~\textbf{utterly} hilarious . \\
Adult&well i 've just been ~\textbf{too busy} .                  &well i 've just been ~\textbf{kinda fun} . & well i 've just been ~\textbf{too busy} .    \\
Adult& these were ~\textbf{common phrases} .    &  these were ~\textbf{common teacher} .  &   these ~\textbf{were common} . \\
	\bottomrule
\end{tabular}
% ... grr ... now i get cold quicker . 
%it was so so totally hilarious 
%same
%these were common ! !

